Online Self-Training for Co-Adaptation in Hierarchical Diffusion Policies

Hierarchical policies decompose language-conditioned long-horizon robotic manipulation into a high-level planner and a low-level controller. However, effective coordination between HL and LL requires that both components operate on compatible subgoal distributions. We propose ORCHID, a self-training framework that enables stable online improvement of hierarchical diffusion policies by aligning planning and control through iterative refinement. By filtering policy samples via environment feedback, ORCHID identifies trajectories where the planner and controller are jointly successful and distills them back into both modules via supervised learning. This process induces a bidirectional co-adaptation: the planner grounds its subgoals in the actual reaching capabilities of the controller, while the controller specializes in the trajectory structures the planner produces. By relying on supervised distillation of filtered on-policy samples, ORCHID avoids the instability typical of online hierarchical gradient-based RL training with diffusion models. On the CALVIN benchmark, ORCHID allows a lightweight, initially weak model to outperform pure offline methods, including a Vision-Language-Action model twice its size.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly state both contributions of the paper: (1) the ORCHID self-training framework for stable iterative improvement of hierarchical diffusion policies from environment feedback, and (2) empirical evidence of bidirectional HL-LL co-adaptation as a driver of performance gains. The scope is explicitly bounded to language-conditioned robotic manipulation. Key assumptions (sparse binary reward, initial offline initialization) and limitations (stalling at near-zero success rates, growing computational cost) are stated in Section~\ref{sec:conclusion}. All quantitative claims in the abstract are supported by the experimental results in Section~\ref{sec:results} and Appendix~\ref{app:results}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations are discussed in Section~\ref{sec:conclusion} (Conclusion) and in dedicated appendix sections. Specifically: (1) computational cost grows with dataset aggregation in ORCHID (vs. constant cost in ORCHID-ft), as analyzed in Appendix~\ref{app_subsec:computational_cost}; (2) self-training stalls when the initial policy achieves near-zero success on a task, as demonstrated for the stack task in the low-data regime (Appendix~\ref{app:low_data}), motivating future work on curriculum learning; (3) the binary success signal, while easy to obtain in simulation, requires a success detector for real-world deployment, discussed in Appendix~\ref{app:real_world}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All information required to reproduce the main results is provided (architecture details in Appendix~\ref{app:archi}, training hyperparameters in Appendix~\ref{app:hyperparmeters}, full training as pseudocode in Appendix~\ref{app:pseudo_code}). Evaluation protocols for both benchmarks are detailed in Section~\ref{sec:exp_setup} and Appendix~\ref{app:envs}. Complete code, data download scripts, training procedure and evaluation are provided in the anonymized repository linked in the abstract, enabling full reproduction of all reported results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: An anonymized repository is provided which details data downloading, training and evaluation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A dedicated Section~\ref{sec:exp_setup} is provided in the main paper describing the evaluation protocols and architecture details, with additional details provided in Appendix~\ref{app:archi} and~\ref{app:envs}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All results are reported as means with standard errors computed over 3 random seeds. Error bars are shown in all figures (shaded regions) and tables ($\pm$ values). When possible (enough samples) statistical significance (t-test p<0.05) is reported. We acknowledge that 3 seeds provides limited statistical power; this is a pragmatic constraint given the substantial computational cost of each evaluation run, which is standard practice for this class of robotics experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Compute requirements are detailed in Appendix~\ref{app:hyperparmeters}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: The research was conducted in accordance with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work presents a foundational training framework for 
language-conditioned robotic manipulation. While we discuss real-world deployment considerations in Appendix~\ref{app:real_world}, the method does not involve personal data, surveillance, or generative models with misuse potential. We do not foresee a direct path to negative societal impacts beyond those inherent to robotics research in general.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer:\answerNA{} % Replace by \answerYes{}, \answerNo{}, or .
    \item[] Justification: The released assets (code, model checkpoints, environment) are robotic manipulation policies trained in simulation. They do not constitute generative models with misuse potential (e.g., image generation, language generation) and do not pose risks that would require access restrictions or safety filters.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: All external assets are cited with their original papers. Licenses are as follows: CALVIN benchmark (MIT License), PyBullet (zlib/libpng License), CLIP (MIT License), Diffusion Policy (MIT License), ACT (MIT License), R3M (MIT License), DINOv2 (Apache 2.0), AVDC (MIT License). All assets are used in accordance with their respective licenses. License information is also documented in the repository README.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The Franka-3Blocks environment introduced in this paper is documented in Appendix~\ref{app:envs}, including task definitions (10 tasks across lift, push, and stack categories), simulator details (PyBullet), demonstration collection procedure, and evaluation protocol. The environment code is released under the MIT License in the anonymized repository. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects. The CALVIN dataset uses teleoperation demonstrations collected by the original CALVIN benchmark authors under their own protocols; we use this data as a fixed offline dataset without collecting new human data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve human subjects research and does not require IRB approval or equivalent review.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core method development in this research does not involve LLMs as any important, original, or non-standard components.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> draft.tex <==
In hierarchical policies, the best training data is not expert data, but data that is consistent with the joint capabilities of the planner and controller.

We restrict our comparisons to offline baselines, as our goal is to improve policies trained from fixed datasets without requiring additional human-annotated data. While online gradient-based RL methods are a natural alternative, applying them to hierarchical policies with diffusion-based components remains an open challenge; instead, we focus on a stable self-training approach based on environment interaction.


While online gradient-based RL methods are a natural alternative for improving policy through interaction with the environment, applying them to hierarchical policies with diffusion-based components remains challenging due to instability arising from non-stationarity across levels \cite{}, which are further exacerbated in diffusion models due to noisy likelihood estimation and high-variance updates \cite{}.


To evaluate the 'search' capacity of our planner, we ablate the guidance scale $g$ during the rollout collection phase. Since $g$ modulates the balance between the conditional and unconditional distributions, it serves as a proxy for search breadth: lower values allow the planner to explore functionally diverse (though potentially noisy) strategies, while higher values collapse the distribution toward the most likely expert-like behavior. We find that a moderate $g$ provides the optimal 'generative search'—diverse enough to find successful trajectories in difficult configurations, yet anchored enough to remain task-relevant.

% Empirically, we provide evidences that \method induces a bidirectional alignment between hierarchical components: \pihl learns to generate subgoals that \pill can actually reach, while \pill simultaneously specializes in generating successful trajectories conditioned on the specific plan structure of \pihl. We show that neither adaptation alone is sufficient, identifying this joint co-adaptation as the key mechanism underlying the method's effectiveness. This alignment, along with the stable improvement loop, significantly improves hierarchical diffusion policies on the Franka-3Blocks and CALVIN benchmarks, even in low-data regimes — ultimately enabling a lightweight model to match or surpass prior offline methods, including a VLA model twice its size pretrained on large-scale data.

% Beyond absolute performance, we show that these gains stem from a bidirectional alignment that emerges between \pihl and \pill over the course of training: \pihl learns to generate subgoals the controller is capable of following, while \pill simultaneously specializes in generating actions to complete the task, conditioned on the specific plans of HL. We show empirically that neither adaptation alone is sufficient. Along with additional data, this joint co-adaptation through the iterative loop is the key mechanism underlying the method's effectiveness.


% $\bullet$ We propose \method, a stable self-training framework for the continual improvement of hierarchical diffusion policies. By leveraging the inherent stochasticity of the diffusion planner as a generative search mechanism, \method enables iterative improvement from environment feedback while avoiding the high variance and instability typically associated with online RL.

% $\bullet$ We characterize a bidirectional alignment mechanism that emerges between the diffusion planner and the controller through iterative self-training: the planner learns to generate more "reachable" subgoals while the controller learns to follow the generated plans to execute the actions leading to success. %, and we show that both adaptations are necessary for the observed performance gains.

% $\bullet$ We provide an empirical evaluation on Franka-3Blocks and the challenging CALVIN benchmark which highlight the advantages of \method regarding sample efficiency and its ability to achieve state-of-the-art performance, outperforming FLOWER \cite{reuss2025flower}, a VLA model twice its size pretrained on large-scale data.


% Hierarchical policies have shown promising results for long-horizon and multitask sequential decision problems. However, a well-known limitation of these models is their instability when trained online, making modern hierarchical methods dependent on large-scale, fixed human datasets. In this work, we improve a diffusion-based hierarchical policy through a self-training process called \method that requires no additional expert demonstrations. \method organizes training into an iterative loop: the stochasticity of the diffusion planner is used as a generative search mechanism to discover successful behaviors from environment feedback, which are then distilled back into both the planner and controller via supervised learning. Our method allows a lightweight, initially weak model to matches or exceeds performance, on the CALVIN benchmark, of a Vision-Language-Action (VLA) model twice its size that is pre- and post-trained purely offline. Furthermore, we show that this improvement stems from a bidirectional alignment between the diffusion planner and the controller: the planner learns to generate subgoals the controller is capable of following, while the controller learns to specialize in the trajectories proposed by the planner.


% While monolithic Vision-Language-Action (VLA) models demonstrate impressive generalization, they typically necessitate extensive pre-training on massive datasets and incur significant inference overhead. To achieve similar multi-task complexity more efficiently, hierarchical policies decompose decision-making into a high-level planner (\pihl) and a low-level controller (\pill).

% To improve diffusion-based hierarchical policies, prior work has attempted to resolve the coupling mismatch between generated plans and \pill capabilities. 


\subsection{Component analysis: \textit{Does \method improve both HL and LL components?}}
\label{subsec:component_analysis}

\begin{table}[!htbp]
\centering
\caption{Cross-evaluation of different HLs, trained on $D_0$ and after 3 iterations of our method using ACT or DP, paired with these LLs on CALVIN LH-MTLC. We report the mean success sequence length (Avg. Len.) and standard error across 3 seeds. HL-LL training pairs are highlighted in \textcolor{blue!60}{blue}, best results in \textbf{bold}.}
{\label{tab:cross_eval}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{c|ccc}
\toprule
\diagbox{LL}{HL} 
& \makecell{HD \\ (iter 0)}
& \makecell{\methodACTft \\ (iter 3)}
& \makecell{\methodft \\ (iter 3)} \\
\midrule
\makecell{\methodACTft \\ (iter 3)} 
& 2.50 \scriptsize{($\pm$ 0.03)} 
& \cellcolor{blue!10} 2.90 \scriptsize{($\pm$ 0.03)}
& \textbf{3.20} \scriptsize{($\pm$ 0.02)} \\
\makecell{\methodft \\ (iter 3)}    
& 2.82 \scriptsize{($\pm$ 0.01)}
& 3.65 \scriptsize{($\pm$ 0.01)} 
& \cellcolor{blue!10} \textbf{3.80} \scriptsize{($\pm$ 0.01)} \\
\bottomrule
\end{tabular}
}
\end{table}

\textbf{HL planner improvement:} To isolate the improvement of \pihlphi, we fix two LL (DP and ACT, both trained with 3 iterations of \methodft) and compare the performance of the resulting policies when combined with different planners: the initial planner (trained on $D_0$), \pihlphi trained with \methodACTft, and \pihlphi trained with \methodft, both for three iterations. Table~\ref{tab:cross_eval} shows the performance of these policies on CALVIN LH-MTLC.
The results demonstrate that both HL fine-tuned with our method (whether paired with ACT or DP during training) outperform the initial HL for both controllers, even when paired with a LL not used during their specific training process. This indicates that in addition to the bidirectional alignment highlighted in the previous section, \pihlphi fine-tuned with our method learns to generate fundamentally better plans that generalize to different \pill. More surprisingly, \pihlphi trained with the DP controller performs better when paired with ACT than the \pihlphi that was actually trained with ACT ($3.20$ vs $2.90$ Avg. Len.). This occurs despite both planners sharing the same architecture, starting from the same \pihlphi initialization trained on $D_0$, and being trained on the same number of data at each iteration. This result demonstrates a synergistic mechanism: being paired with a stronger initial controller (DP) leads to the collection of higher-quality data, which in turn results in a more capable and generalizable HL.
 
\textbf{LL controller improvement:} To evaluate the improvement of \pillpsi, we utilize ground truth (GT) subgoals extracted from the CALVIN MTLC validation set. Table~\ref{tab:oracle} compares the performance of hierarchical agents guided by GT subgoals with the \pillpsi trained solely on $D_0$ against the \pillpsi fine-tuned with three iterations of \method. We observe that the \pillpsi fine-tuned with our method outperforms the one trained only on $D_0$. Since this improvement occurs under GT guidance, it is independent of \pihlphi’s performance, thereby demonstrating the intrinsic improvement of \pillpsi.

\begin{table}[htpb]
\centering
\caption{Cross-evaluation of HD policies with LLs trained solely on $D_0$ (iter 0) and trained with 3 iterations of \method (iter 3), guided by ground truth (GT) subgoals, and the respective HL with and without replanning. Results are reported as mean success rates and standard errors across 3 seeds on CALVIN MTLC.}
\label{tab:oracle}
\small
\begin{tabular}{c|c|c}
\toprule
HL & LL & SR (\%) \\
\midrule

GT 
    & \multirow{4}{*}{HD (iter 0)} 
    & 90.0 ($\pm$ 0.1) \\

\makecell{HD (iter 0) \\ w/o replan. } 
    &  
    & 83.3 ($\pm$ 0.1) \\

HD (iter 0)
    &  
    & 89.8 ($\pm$ 0.5) \\

\midrule

GT 
    & \multirow{4}{*}{\method (iter 3)} 
    & 91.2 ($\pm$ 0.5) \\

\makecell{\method (iter 3) \\ w/o replan. } 
    &  
    & 92.1 ($\pm$ 0.3) \\
    
\method (iter 3) 
    &  
    & 95.2 ($\pm$ 0.2) \\

\bottomrule
\end{tabular}
\end{table}

% \subsection{Metrics}

% \textbf{Reachability error.}
% In order to evaluate to what extend Hl generetas plans that LL is able to reach, we introduce the \textit{reachability error} define the \emph{reachability error} as the expected observation-space distance between the conditioning subgoals and the states actually reached by the controller:
% $$
% \mathcal{F}(\pi^{HL}_\phi, \pi^{LL}_\psi) = \mathbb{E}_{\substack{(s_0, l) \sim \rho_0 \times L \\ \hat{\zeta} \sim \pi^{HL}_\phi(\cdot \mid O(s_0), g) \\ \tau \sim \pi^{LL}_\psi(\cdot \mid \hat{\zeta}, O(s_0))}} \left[ \frac{1}{M} \sum_{i=1}^{M} d\!\left(O(s_{t_i}),\, \hat{o}_i\right) \right]
% $$
% where $s_{t_i}$ is the true environment state reached at step $t_i$, and $d$ is a distance metric over observation space. Defining a robust distance metric $d$ over visual observations is non-trivial, as no single representation perfectly captures task-relevant configurations while remaining invariant to visual noise. To ensure a comprehensive assessment, we evaluate reachability error $\mathcal{F}$ using $l2$ distance across three complementary embedding spaces: pixel-space for raw scene sensitivity, R3M~\citep{} for robotic-centric features learned from human manipulation, and DINOv2~\citep{} for broad semantic and structural scene understanding. Reporting across these divergent metrics ensures that observed improvements reflect genuine physical reachability rather than artifacts of a specific representation, with consistent trends providing high-confidence evidence of state proximity.

% \textbf{Expected return.} 
% Crucially, low reachability error is necessary but not sufficient for task success due to the partial observability inherent in visual subgoals. Because $\hat{o}_i \in \mathbb{R}^{3 \times H \times W}$ lacks full state information—such as end-effector velocities, applied forces, or precise continuous orientations obscured by occlusions—minimizing $\mathcal{F}$ does not guarantee that the underlying physical state $s_{t_i}$ is viable for subsequent task progression. Even if a plan is geometrically reachable in image space, the controller's resulting action distribution must still solve the underlying RL problem. Therefore, we rely on the expected task reward obtained by $\pi^{LL}_\psi$ when conditioned on the specific trajectory structures induced by $\pi^{HL}_\phi$.

% In the rest of this work, we use $\mathcal{F}$ and $J$ to characterize the respective adaptation of each component. We say that $\pi^{HL}_1$ is more \textit{adapted} to a controller $\pi^{LL}$ than $\pi^{HL}_2$ if $\mathcal{F}(\pi^{HL}_1, \pi^{LL}) < \mathcal{F}(\pi^{HL}_2, \pi^{LL})$, and that $\pi^{LL}_1$ is more \emph{aligned} with a planner $\pi^{HL}$ than $\pi^{LL}_2$ if $J(\pi^{HL}, \pi^{LL}_1) > J(\pi^{HL}, \pi^{LL}_2)$. 


% \textbf{Franka-3Blocks environment:} To highlight the benefits of our method for improving hierarchical diffusion (HD) policies, we evaluate versions of \method in an environment composed of 10 manipulation tasks defined by fixed language instructions. In order to construct the initial training set $D_0$, we use a hand-crafted expert with access to privileged environment and robot state information. The policies are evaluated on 100 randomly sampled settings per tasks.

% \textbf{CALVIN environment:} To evaluate our method against baselines, we train our policy with the different \method variants in the CALVIN environment~\citep{mees2022calvin}. This environment contains 34 language-conditioned manipulation tasks and provides an initial training set $D_0$ collected through human teleoperation. We consider the $D \rightarrow D$ setting, where the agent sees the same environment at train and test. Despite being the in-distribution split, $D\rightarrow D$ is empirically the hardest (see CALVIN leaderboard \citep{mees2022calvin}) as it features the scarcest training dataset, making it the most stringent setting for evaluating gains from self-training under limited supervision. Each task $l$ has 10 textual goals $g$ in training, while evaluation uses unseen textual goals. We consider two evaluation protocols: \textbf{Multi-Task Language-Conditioned (MTLC):} complete each task in 30 unseen fixed settings and textual goals. This protocol aims to evaluate generalization to contexts unseen in $D_0$. \textbf{Long-Horizon MTLC (LH-MTLC):} complete 5 consecutive tasks, starting from 1000 contexts sampled from the fixed environment reset distribution with unseen textual goals. This protocol is more challenging and evaluates the capacity of the policy to maintain performance over long sequences.

% In practice, $J$ is estimated as the success rate (SR) on individual tasks, while in LH-MTLC, the average number of consecutively completed instructions (Avg. Len.) serves as a proxy to measure how long the policy maintains high $J$ across a sequence of tasks. Further details on the environments can be found in Appendix~\ref{app:envs}.

% \subsection{Baselines}
% \label{subsec:baselines}

% We compare the performance of our hierarchical diffusion (HD) policy trained solely on the fixed initial dataset $D_0$ (corresponding to iteration 0) with the policy after up to 3 iterations of \method and \methodft using either ACT or DP controllers. We further compare our approach against hierarchical policies from prior work, all trained from scratch on the CALVIN dataset. Each of these baselines represents a distinct strategy for improving hierarchical agents by aligning \pihlphi and  \pillpsi (see Figure~\ref{fig:main}(a)(b)(c) with further details in Appendix~\ref{app:baselines}):

% $\bullet$ Independent HL--LL training: SuSIE~\citep{black2023Susie}.

% $\bullet$ Alignment through a "glue" model based on estimated task progress: TaKSIE~\citep{kang2025taksie}.

% $\bullet$ Alignment through shared representations: HULC~\citep{mees2022HULC} and MDT~\citep{reuss2024MDT}, which use an autoregressive \pihl, and LDC~\citep{zhang2024LDC}, which uses a diffusion-based \pihl.

% We further compare our method to FLOWER~\citep{reuss2025flower} which is the current SOTA on all CALVIN benchmarks. However, while the previous baselines are trained from scratch, FLOWER is a 950M parameter VLA that leverages a VLM pre-trained on internet-scale data, itself pre-trained on 250k robotic trajectories and then fine-tuned on the same initial dataset as the rest of the baselines.


% \subsection{Self-training for language model reasoning} Expert Iteration~\citep{Anthony2017ExpertIteration} first demonstrated that models can bootstrap performance by filtering their own sampled outputs and distilling successes back into the policy. This principle has since proven highly effective in LLMs: STaR~\citep{zelikman2022star} improves chain-of-thought reasoning by retaining only correct self-generated rationales, ReST~\citep{gulcehre2023reinforcedselftrainingrestlanguage} iteratively grows a filtered replay dataset, and SPIN~\citep{chen2024selfplayfinetuningconvertsweak} shows that self-play distillation converts weak models into strong ones without additional human demonstrations. Most recently, DeepSeek-R1~\citep{guo2025deepseek} demonstrates that iterative self-training can produce reasoning capabilities competitive with much larger supervised models. A common theme across these works is that supervised distillation of filtered on-policy samples is more stable than direct gradient-based RL fine-tuning while achieving similar or even superior performances~\citep{havrilla2024teachinglargelanguagemodels}. This property makes self-training particularly attractive for architectures where policy gradients are unreliable, such as diffusion-based hierarchical planners, which directly motivates the core update mechanism of \method.

% \subsection{Hierarchical policies for language-conditioned manipulation}

% The HL-LL coupling problem has been recognized implicitly across prior work, though rarely addressed as a unified challenge. TaKSIE \citep{kang2025taksie} and HL-Glue \citep{hatch2024ghilglue} introduce an intermediate "glue" model to perform subgoal selection based on estimated task progress reflecting LL's preferences (\figurename~\ref{fig:main}(b)). While effective, this approach requires frequent replanning and additional inference-time optimization, increasing latency and system complexity. HIP \citep{ajay2023HIP} uses an auxiliary model during training to regularize a diffusion HL toward LL’s preferences, but this direct regularization can induce high variance and training instability.

% Other methods enforce coupling through joint representations, either via shared network layers (MDT \citep{reuss2024MDT}) or by planning directly in the visual embedding space of LL (LDC \citep{zhang2024LDC}; LDP \citep{xie2025ldp}). However, learning a representation space that simultaneously satisfies the divergent requirements of planning—grounding semantic instructions into spatial modifications—and control—requiring detailed object representations—remains a significant challenge. Furthermore, these methods rely on a single offline training stage, fundamentally limiting their ability to improve beyond the initial dataset coverage. Critically, none of these approaches enable online co-adaptation between planner and controller from environment feedback. In contrast, our approach drives a bidirectional co-adaptation between HL and LL through iterative on-policy refinement, without introducing auxiliary models, shared latent constraints, or gradient-based coordination losses.

% \subsection{Fine-tuning diffusion-based and hierarchical policies with environment feedback}

% Fine-tuning policies from environment feedback is a promising avenue to push manipulation capabilities beyond offline supervised learning \citep{julian2020stoplearningeffectivenessfinetuning, hu2024flareachievingmasterfuladaptive, tang2024deepreinforcementlearningrobotics}. However, traditional reinforcement learning is highly unstable when applied to hierarchical policies \citep{levy2019HRL, make2022HRL_survey_challenges}, making convergence difficult in long-horizon tasks \citep{nachum2018dataefficienthierarchicalreinforcementlearning}. This challenge is amplified for diffusion-based policies, as gradient-based fine-tuning must propagate through multi-step stochastic denoising processes \citep{ren2024diffusionpolicypolicyoptimization}. Existing methods for fine-tuning diffusion models either require dense rewards \citep{fan2023dpokreinforcementlearningfinetuning, black2024ddpo} or rely on preference datasets \citep{wallace2023diffusionmodelalignmentusing, yang2024D3PO}, neither of which is typically available in language-conditioned manipulation. An alternative avenue uses learned world models as surrogate environments for offline policy fine-tuning~\citep{chandra2025diwa, han2026wam}, avoiding real environment interaction entirely. However, these methods target flat diffusion policies and require training a separate world model, whereas \method improves 
% hierarchical policies directly from sparse binary environment 
% feedback without additional learned components. While SAILOR \citep{jain2025smoothseaskilledsailor} and DifNav \citep{shi2025daggerdiffusionnavigationdagger} progressively improve diffusion policies using iterative search, they focus on flat diffusion policies where a single component is optimized end-to-end. Extending iterative refinement to hierarchical policies introduces the additional challenge of jointly improving two interdependent components, planner and controller.

% Our framework extends iterative refinement to hierarchical diffusion policies, fine-tuning directly from sparse, binary environment feedback. By utilizing feedback-based filtering instead of direct policy gradients, \method provides a stable mechanism to concurrently optimize planning and control, unlocking continual improvement without reliance on external expert. %To our knowledge, no prior work enables stable online improvement of hierarchical diffusion policies using only sparse binary feedback, a gap that \method directly addresses.

% \subsection{Architectures}

% The high-level planner is a lightweight diffusion 3D CNN U-Net (based on AVDC~\citep{ko2023AVDC}) which generate subgoal sequences conditioned on the initial observation $o_0$ and a frozen CLIP~\citep{radford2021CLIP} embedding of the textual goal $g$. For the main experiments, we use the DDPM~\citep{ho2020DDPM} noise scheduler for both training and inference, while we investigate the use of DDIM~\citep{song2022DDIM} to reduce inference overhead in Appendix~\ref{app:ddpm_vs_ddim}. For the low-level controller, we evaluate two architectures adapted for goal-conditioning: a Diffusion Policy (DP)~\citep{chi2024diffusionpolicyvisuomotorpolicy} and an Action Chunk Transformer (ACT)~\citep{zhao2023learningfinegrainedbimanualmanipulation}. By default, \method uses the DP controller, while the ACT variant is denoted as \methodACT. Further architectural details and hyperparameters are provided in Appendix~\ref{app:archi}.

% Task success does not increase, however. The issue can be explained by the partial observability in the subgoal representation~\citep{leveraging_sequentiality}: a visual subgoal can correspond to many distinct underlying states, the subgoal defines \emph{where} to be visually, but not \emph{how} to get there to complete the task, leaving the execution trajectory underspecified. $LL_{D_0}$ has learned to generate trajectories (e.g. approach or grasp orientations) conditioned on human teleoperation subgoals, not on the distribution induced by $\text{HL}_{R_1}$. This suggest that subgoals reachability is necessary but not sufficient; the controller must also adapt to the specific trajectory structures the planner produces, in order to translate reaching subgoals into achieving the task.


% This suggests that geometric reachability is necessary but insufficient for success. $\text{LL}_{D_0}$, trained strictly on expert demonstrations, lacks the specific behavioral nuances required to translate the planner's reachable subgoals into functional manipulation.

